Control Under Action-Dependent Markov Packet Drops: An Event-Triggered Approach

In this paper, we consider the problem of second moment stabilization of a scalar linear plant with process noise. We assume that the sensor must communicate with the controller over an unreliable channel, whose state evolves according to a Markov chain, with the transition matrix on a timestep depending on whether there is a transmission or not on that timestep. Under such a setting, we propose an event-triggered transmission policy which meets the objective of exponential convergence of the second moment of the plant state to an ultimate bound. Furthermore, we provide upper bounds on the transmission fraction of the proposed policy. The guarantees on performance and transmission fraction are verified using simulations.

==> macros.tex <==
% macro tex file for current manuscript
% RATIONALE:
% \macro{option used}{main argument}
% \macro{}{main argument} % optional argument not used
%
% this helps in recycling a lot of the code.

% these macros need amsmath package
\RequirePackage{amsmath}
% for the occassonal oddball case
\usepackage{cprotect}

% script to detokenize # symbol
\makeatletter
\def\ifemptyarg#1{%
	\if\relax\detokenize{#1}\relax % H. Oberdiek
	\expandafter\@firstoftwo
	\else
	\expandafter\@secondoftwo
	\fi}
\makeatother

% POLICY SYMBOLS
\newcommand{\etpol}[1][]{
	\ifemptyarg{#1}
	{\mathcal{T}^{D}_{et}}
	{\mathcal{T}^{#1}_{et}}
}
\newcommand{\nompol}[1][]{
	\ifemptyarg{#1}
	{\mathcal{T}^{D}_k}
	{\mathcal{T}^{#1}_k}
}

% EXPECTATION MACRO
\newcommand{\expect}[2]{
	\ifemptyarg{#1}
	{\mathbb{E} \left[ #2 \right]}
	{\mathbb{E}_{#1} \left[ #2 \right]}
}

% EVENT-TRIGGERED POLICY RELATED MACROS
\newcommand{\exsep}{ \, \vert \,}
\newcommand{\tkd}{\Mcal{T}^D_k}
\newcommand{\G}[2]{\Mcal{G}_{#1}^{#2}}
\newcommand{\J}[2]{\Mcal{J}_{#1}^{#2}}
\newcommand{\gdk}{\mathcal{G}_k^D}
\newcommand{\jdk}{\mathcal{J}_k^D}
\newcommand{\mb}[1]{\mathbf{#1}}
\newcommand{\prob}{\text{Pr}}
\newcommand{\et}{\mathbb{E}_{\mathcal{T}_\mathcal{E}}}
\newcommand{\jdsj}{\mathcal{J}^D_{S_j}}
\newcommand{\ti}[1]{\tilde{#1}}

% CHANNEL AND STATE VARIABLE MACROS
\newcommand{\tk}{t_k}
\newcommand{\rk}{r_k}
\newcommand{\pone}{\mathbf{P}_1}
\newcommand{\pzero}{\mathbf{P}_0}
\newcommand{\ponee}{\mathbf{P}_1\mathbf{E}}

% Transmission fraction macros
\newcommand{\czero}{\Mcal{C}^{(0)}}
\newcommand{\cone}{\Mcal{C}^{(1)}}
\newcommand{\horzero}{\Delta^{(0)}}
\newcommand{\horone}{\Delta^{(1)}}
\newcommand{\horizon}{\Delta}

% BORROWED FROM PREVIOUS PAPERS
\newcommand{\real}{\ensuremath{\mathbb{R}}}
\newcommand{\intpos}{{\mathbb{N}}}
\newcommand{\intnonneg}{{\mathbb{N}}_0}
\newcommand{\ldef}{:=}
\newcommand{\rdef}{=:}
\newcommand{\abar}{\bar{a}}
\newcommand{\Sj}{S_j}
\newcommand{\Sjnext}{S_{j+1}}

% PREVIOUS PAPERS - OPERATOR DECLARATIONS
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

% SET CONTAINERS
\newcommand{\integers}{{\mathbb{Z}}}
\newcommand{\until}[1]{\{1,\dots,{#1}\}}
\newcommand{\intrangecc}[2]{[#1, #2]_\integers}
\newcommand{\intrangeoo}[2]{(#1, #2)_\integers}
\newcommand{\intrangeoc}[2]{(#1, #2]_\integers}

% FUNCTION COMMANDS
\newcommand{\infsum}[1]{
	\ifemptyarg{#1}
	{(\mathbf{I}-\mathbf{P}_1\mathbf{E})^{-1}}
	{(\mathbf{I}-{#1}\mathbf{P}_1\mathbf{E})^{-1}}}
\newcommand{\infsums}[1]{(\mathbf{I}-{#1}^2\mathbf{P}_1\mathbf{E})^{-1}}
\newcommand{\tpolicy}{\mathcal{T}}
\newcommand{\svecspace}{\mathbb{P}^n}
\newcommand{\bM}{\bar{M}}

% TRANSMISSION FRACTION RELATED MACROS 
% \newcommand{\ltstar}{\Lambda^{(\theta)}_*}
% \newcommand{\ltsstar}{\Lambda^{(\theta)}_{**}}
\newcommand{\llow}{\Lambda_1}
\newcommand{\lhi}{\Lambda_2}
\newcommand{\tf}[1]{\mathcal{F}^{#1}}
\newcommand{\tfs}[1]{\mathcal{F}_{#1}}
\newcommand{\sx}{\mathcal{X}}
\newcommand{\tpart}{\Delta^{(j)}_*}
\newcommand{\ttpart}{\Delta^{(j)}_{**}}

% DOT AFTER FINISHING REMARKS, ETC.
\newcommand{\bulletend}{\relax\ifmmode\else\unskip\hfill\fi\hbox{$\bullet$}}

% Another bunch of macros
\newcommand{\Mcal}[1]{\mathcal{#1}}
\newcommand{\tth}[1]{#1^\text{th}}
\newcommand{\id}{\mathbf{I}}
\newcommand{\canbasis}[1]{\pmb{\delta}_{#1}}
\newcommand{\specrad}[1]{\mathbf{\rho} \left( #1 \right)}
\newcommand{\xkp}{\hat{x}_k^+}
\newcommand{\pk}{\mathbf{p}_k}
\newcommand{\dt}{\mathbf{d}^T}
\newcommand{\psj}{\mathbf{p}_{S_j}}
\newcommand{\gsj}{\gamma_{S_j}}
\newcommand{\gsl}{\gamma_{S_l}}
\newcommand{\hx}{\hat{x}}
\newcommand{\pz}{p^{(0)}}
\newcommand{\po}{p^{(1)}}
\newcommand{\cstate}{\gamma_k}
\newcommand{\Rk}{R_k}
\newcommand{\Ik}{I_k}
\newcommand{\Om}[1]{\Omega_{#1}}
\newcommand{\onevec}{\mathbf{1}}

% Some more macros
\newcommand{\tfsxText}{transmission fraction up to state $\sx$\ } % text macro
\newcommand{\tfsxTextCap}{Transmission fraction up to state $\sx$\ } % text macro
\newcommand{\matrixterms}[2]{\mb{\Pi}_{#1}(#2)}
